An Equivariant Pretrained Transformer for Unified 3D Molecular Representation Learning

Pretraining on a large number of unlabeled 3D molecules has showcased superiority in various scientific applications. However, prior efforts typically focus on pretraining models in a specific domain, either proteins or small molecules, missing the opportunity to leverage cross-domain knowledge. To mitigate this gap, we introduce Equivariant Pretrained Transformer (EPT), an all-atom foundation model that can be pretrained from multiple domain 3D molecules. Built upon an E(3)-equivariant transformer, EPT is able to not only process atom-level information but also incorporate block-level features (e.g. residuals in proteins). Additionally, we employ a block-level denoising task, rather than the conventional atom-level denoising, as the pretraining objective. To pretrain EPT, we construct a large-scale dataset of 5.89M entries, comprising small molecules, proteins, protein-protein complexes, and protein-molecule complexes. Experimental evaluations on downstream tasks including ligand binding affinity prediction, protein property prediction, and molecular property prediction, show that EPT significantly outperforms previous state-of-the-art methods in the first task and achieves competitively superior performance for the remaining two tasks. Furthermore, we demonstrate the potential of EPT in identifying small molecule drug candidates targeting 3CL protease, a critical target in the replication of SARS-CoV-2. Among 1,978 FDA-approved drugs, EPT ranks 7 out of 8 known anti-COVID-19 drugs in the top 200, indicating the high recall of EPT. By using Molecular Dynamics (MD) simulations, EPT further discoveries 7 novel compounds whose binding affinities are higher than that of the top-ranked known anti-COVID-19 drug, showcasing its powerful capabilities in drug discovery.

==> tables/ec.tex <==
\begin{table}[htbp]
\centering
\caption{Results on Enzyme Commission number prediction (EC) and mutation stability prediction (MSP). The best scores are marked in \textbf{bold} and the second best \underline{underlined}.}
\label{tab:ec}
% \scalebox{0.8}{
\begin{tabular}{llcccc}
\toprule
                              & \multirow{2}{*}{Model} & \multicolumn{2}{c}{EC}          &  & MSP         \\ \cmidrule{3-4} \cmidrule{6-6} 
                              &                        & F1 Max         & AUPRC          &  & AUROC       \\ \midrule
\multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}w/o \\ Pretrain\end{tabular}} & GCN                    & 0.320          & 0.319          &  & 0.621       \\
                              & Atom3D-CNN             & -              & -              &  & 0.574       \\
                              & Atom3D-ENN             & -              & -              &  & 0.574       \\
                              & GVP                    & 0.489          & 0.482          &  & \underline{0.680} \\
                              & GearNet                & 0.730          & 0.751          &  & -           \\
                              & GearNet-Edge           & \underline{0.810}& \underline{0.835}&  & 0.633       \\
                              & EPT (ours)             & \textbf{0.823} & \textbf{0.844} &  &  \textbf{0.700}           \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}w/ \\ Pretrain\end{tabular}}  & LM-GVP                 & 0.664          & 0.710          &  & -           \\
                              & ProtBERT-BFD           & 0.838          & 0.859          &  & -           \\
                              & GearNet-Edge           & \textbf{0.874} & \textbf{0.892} &  & \underline{0.646} \\
                              & EPT (ours)             & \underline{0.858}    & \underline{0.871}    &  &         \textbf{0.741}    \\ \bottomrule
\end{tabular}
% }
\end{table}

==> tables/ec_ori.tex <==

\section{More Results on Protein Tasks}
\label{app:prot}

\begin{table*}[htbp]
\centering
\begin{tabular}{ccccccc}
\midrule
\multirow{2}{*}{}                 & \multirow{2}{*}{Model}      & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pretraining\\ Dataset (Size)\end{tabular}} & \multirow{2}{*}{EC} & \multicolumn{3}{c}{GO} \\ \cline{5-7} 
                                  &                             &                                                                                       &                     & BP     & MF    & CC    \\ \midrule
\multirow{16}{*}{w/o pretraining} & CNN                         & -                                                                                     & 0.545               & 0.244  & 0.354 & 0.287 \\
                                  & ResNet                      & -                                                                                     & 0.605               & 0.280  & 0.405 & 0.304 \\
                                  & LSTM                        & -                                                                                     & 0.425               & 0.225  & 0.321 & 0.283 \\
                                  & Transformer                 & -                                                                                     & 0.238               & 0.264  & 0.211 & 0.405 \\ \cline{2-7} 
                                  & GCN                         & -                                                                                     & 0.320               & 0.252  & 0.195 & 0.329 \\
                                  & GAT                         & -                                                                                     & 0.368               & 0.284  & 0.317 & 0.385 \\
                                  & GVP                         & -                                                                                     & 0.489               & 0.326  & 0.426 & 0.420 \\
                                  & 3DCNN\_MQA                  & -                                                                                     & 0.077               & 0.240  & 0.147 & 0.305 \\
                                  & GraphQA                     & -                                                                                     & 0.509               & 0.308  & 0.329 & 0.413 \\
                                  & New IEConv                  & -                                                                                     & 0.735               & 0.374  & 0.544 & 0.444 \\
                                  & GearNet                     & -                                                                                     & 0.730               & 0.356  & 0.503 & 0.414  \\
                                  & GearNet-IEConv              & -                                                                                     & 0.800               & 0.381  & 0.563 & 0.422 \\
                                  & GearNet-Edge                & -                                                                                     & 0.810               & 0.403  & 0.580 & 0.450 \\
                                  & GearNet-Edge-IEConv         & -                                                                                     & 0.810               & 0.400  & 0.581 & 0.430 \\ \cline{2-7} 
                                  & EPT (ours)                  & -                                                                                     & 0.716               & 0.340  & 0.472 & 0.416 \\
                                  & EPT-IEConv (ours)           & -                                                                                     & 0.823               & 0.384  & 0.572 & 0.444 \\ \midrule
\multirow{8}{*}{w/ pretraining}   & DeepFRI                     & Pfam (10M)                                                                            & 0.631               & 0.399  & 0.465 & 0.460 \\
                                  & ESM-1b                      & UniRef50 (24M)                                                                        & 0.864               & 0.452  & 0.657 & 0.477 \\
                                  & ProtBERT-BFD                & BFD (2.1B)                                                                            & 0.838               & 0.279  & 0.456 & 0.408 \\
                                  & LM-GVP                      & UniRef100 (216M)                                                                      & 0.664               & 0.417  & 0.545 & 0.527 \\
                                  & GearNet-Multiview Constrast & AlphaFoldDB (805K)                                                                    & 0.874               & 0.490  & 0.654 & 0.488 \\ \cline{2-7} 
                                  & EPT-mol (ours)              &                                                                                       &                     &        &       &       \\
                                  & EPT-prot (ours)             &                                                                                       &                     &        &       &       \\
                                  & EPT-hybrid (ours)           &                                                                                       & 0.858               & 0.411  & 0.600 & 0.456 \\ \midrule
\end{tabular}
\end{table*}

==> tables/model_abl.tex <==
\begin{table}[b]
\caption{Evaluation of each proposed component on the QM9 dataset. Best results are marked in \textbf{bold}.}
% \resizebox{0.95\linewidth}{!}{
\begin{tabular}{l|cccc|cc}
\addlinespace[5pt]
\toprule

\multicolumn{1}{l|}{} & \begin{tabular}[c]{@{}c@{}}Block \\ Emb.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Dist. \\ Attn.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Edge \\ Attn.\end{tabular} & \multicolumn{1}{c|}{FFN}  & $\epsilon_{\text{HOMO}}$         & $\epsilon_{\text{LUMO}}$         \\ \midrule
Ours                  & \checkmark                             & \checkmark                              & \checkmark                             & \checkmark & \textbf{19.2}         & \textbf{17.4}         \\ 

        \midrule
        \addlinespace[-0.1pt]
        % \rowcolor{gray!30}
        \multicolumn{7}{c}{\textit{Block-level Embeddings}} \\
        \addlinespace[-2pt]
        \midrule
Atom Emb. Only        &                                                       & \checkmark                              & \checkmark                             & \checkmark & 19.5         & 17.6         \\
        \midrule
        \addlinespace[-0.1pt]
        % \rowcolor{gray!30}
        \multicolumn{7}{c}{\textit{Attention Mechanism}} \\
        \addlinespace[-2pt]
        \midrule
Standard Attn.        & \checkmark                             &                                                        &                                                       & \checkmark & 23.2         & 20.4         \\
w/ Dist. Attn.        & \checkmark                             & \checkmark                              &                                                       & \checkmark & 22.3         & 19.4         \\
w/ Edge Attn.         & \checkmark                             &                                                        & \checkmark                             & \checkmark & 20.4         & 17.7         \\
        \midrule
        \addlinespace[-0.1pt]
        % \rowcolor{gray!30}
        \multicolumn{7}{c}{\textit{Feed Forward Network}} \\
        \addlinespace[-2pt]
        \midrule
w/o FFN               & \checkmark                             & \checkmark                              & \checkmark                             &                           & 28.2         & 26.6         \\ \bottomrule
\end{tabular}
\label{tab:model_abl}
% }
\end{table}

==> tables/pretrain_abl.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{Comparison on the LBA and QM9 results from different pretraining settings. Best results are marked in \textbf{bold}.}
\centering
% \resizebox{0.8\linewidth}{!}{
\begin{tabular}{lccccc}
\addlinespace[5pt]
\toprule
Pretraining & \multicolumn{2}{c}{PCC$\uparrow$}     &    & \multicolumn{2}{c}{MAE$\downarrow$}       \\ \cmidrule{2-3}\cmidrule{5-6}
Setting                                  & ID30     & ID60    & & $\epsilon_{\text{HOMO}}$         & $\epsilon_{\text{LUMO}}$        \\ \midrule
-                                          & 0.604          & 0.777   &       & 19.2          & 17.4          \\
        \midrule
        \addlinespace[-0.1pt]
        % \rowcolor{gray!30}
        \multicolumn{6}{c}{\textit{Dataset Domain}} \\
        \addlinespace[-2pt]
        \midrule
Molecule Only & 0.627 & 0.791 & & 17.5 & 15.5 \\
Protein Only & 0.628 & 0.805 & & 18.9 & 16.7 \\ 
        \midrule
        \addlinespace[-0.1pt]
        % \rowcolor{gray!30}
        \multicolumn{6}{c}{\textit{Denoising Strategy}} \\
        \addlinespace[-2pt]
        \midrule
$\gL_{\text{atom}}  $                                                 & 0.613          & 0.807          & & 17.1          & 14.6          \\
$\gL_{\text{block-T}}$                                                & 0.636          & 0.817          & & 17.5          & 14.8          \\ \midrule
Ours                                              & \textbf{0.643} & \textbf{0.822} & & \textbf{16.2} & \textbf{14.1} \\ \bottomrule
\end{tabular}
\label{tab:target}
% }
\end{table}

